FATCAT: Fault Injection Attacks Targeting Chip-level Alignment

Model alignment is the primary safety and security mechanism for enforcing refusal of malicious prompts in modern foundation models; yet, existing adversarial evaluations implicitly assume underlying hardware integrity. In this paper, we present FATCAT, the first physical fault-injection attacks capable of eliminating refusal in modern large language and vision-language models. Specifically, we present a non-invasive electromagnetic (EM) fault injection attack targeting GPU-accelerated Systems-on-Chip with physical access, requiring neither software execution privileges nor model-layer access. By leveraging an autonomous Radio Frequency (RF) side-channel trigger to synchronize EM faults to the prompt prefill phase, the attack corrupts safety-critical memory transactions across off-chip LPDDR5 DRAM and on-chip LPDDR physical interfaces without crashing the system while preserving model coherence. Evaluated on an NVIDIA Jetson Orin Nano and AGX Thor running Llama 3.2 1B and Gemma 3 1B, localized physical faults reliably force models to fulfill restricted requests, demonstrating that model-level alignment provides no robust security guarantees without hardware-level fault tolerance. Finally, we demonstrate the physical-world consequences of this vulnerability on an active 6-DoF robotic manipulator controlled by a SmolVLA vision-language-action policy. Our attack silently corrupts the model forcing the arm into abrupt, hazardous lunges; in two instances the robotic arm attempted to pinch the paper author -- proving that hardware faults can directly translate into real physical harm.

==> tex/overview_titlepage.tex <==
\begin{tikzpicture}[x=1pt, y=1pt, line cap=round, line join=round,
    heading/.style={rounded corners=5.2pt, inner xsep=7pt, inner ysep=0pt, minimum height=10.4pt,
                    text=white, font=\fontsize{7}{8}\selectfont\bfseries}]
  \pgfmathsetmacro{\W}{\textwidth}                   %
  \pgfmathsetmacro{\pad}{7}                          %
  \pgfmathsetmacro{\gap}{22}                         %
  \pgfmathsetmacro{\sp}{6}                           %
  \pgfmathsetmacro{\cap}{12.5}                       %
  \pgfmathsetmacro{\fw}{(\W-2.8-2*\pad-2*\gap)/3}    %
  \pgfmathsetmacro{\fh}{\fw*0.6669}                  %
  \pgfmathsetmacro{\HB}{2*\sp+\cap+\fh}              %
  \pgfmathsetmacro{\ya}{\sp+\cap}                    %
  \pgfmathsetmacro{\cy}{\ya+0.5*\fh}                 %
  \pgfmathsetmacro{\Hd}{\W*0.40777}                  %
  \pgfmathsetmacro{\yA}{\HB+19.8}                    %
  \pgfmathsetmacro{\yT}{\yA+0.990*\Hd}               %
  \useasboundingbox (0,0) rectangle (\W,\yA+\Hd);

  \node[anchor=south west, inner sep=0pt, outer sep=0pt] at (0,\yA)
    {\includegraphics[width=\W pt]{img/setup/attack_overview_diagram_wide.pdf}};
  \node[heading, fill=black!80, anchor=south west] (how) at (1.4,\yT+2.4) {\textls[90]{HOW IT WORKS}};
  \draw[gray!60, line width=0.6pt, line cap=butt] ([xshift=4pt]how.east) -- (\W-1.4,0 |- how.east);

  \fill[black!90, rounded corners=4pt] (1.4,0) rectangle (\W-1.4,\HB);
  \foreach \k in {0,...,32} {                        %
    \pgfmathsetmacro{\hx}{1.4+6+\k*(\W-2.8-12-6.4)/32}
    \fill[white, rounded corners=0.9pt] (\hx,1.5) rectangle (\hx+6.4,4.6);
    \fill[white, rounded corners=0.9pt] (\hx,\HB-4.6) rectangle (\hx+6.4,\HB-1.5);
  }
  \node[heading, fill=filmred, anchor=south west] (cam) at (1.4,\HB+2.4)
    {\textbullet\kern3pt\textls[90]{CAUGHT ON CAMERA}};
  \node[heading, anchor=south east, fill=white, draw=filmred, line width=0.8pt, text=filmred,
        inner xsep=6pt] (watch) at (\W-1.8,\HB+2.4)
    {\href{\videoaddress}{\hspace{8pt}\textcolor{filmred}{\textls[90]{WATCH THE CLIPS}}}};
  \fill[filmred] ([xshift=6pt,yshift=-3pt]watch.west) -- ++(0,6) -- ++(5.2,-3) -- cycle;
  \draw[filmred, line width=0.6pt, line cap=butt] ([xshift=4pt]cam.east) -- ([xshift=-4pt]watch.west |- cam.east);
  \foreach \i/\img/\bc/\bw/\tm/\cc/\what in {
      0/clip1_a_reach/white/0.9/{\phantom{+}0.00\,s}/white/OPERATOR REACHES IN,
      1/clip1_b_rear/filmred/1.4/{+0.36\,s}/filmyellow/THE ARM REARS UP,
      2/clip1_c_lunge/filmred/1.4/{+0.56\,s}/filmyellow/LUNGES AT THE HAND} {
    \pgfmathsetmacro{\xa}{1.4+\pad+\i*(\fw+\gap)}
    \begin{scope}
      \clip[rounded corners=2.6pt] (\xa,\ya) rectangle (\xa+\fw,\ya+\fh);
      \node[anchor=south west, inner sep=0pt, outer sep=0pt] at (\xa,\ya)
        {\includegraphics[width=\fw pt, height=\fh pt]{img/robot_frames/\img.jpg}};
    \end{scope}
    \draw[\bc, line width=\bw pt, rounded corners=2.6pt] (\xa,\ya) rectangle (\xa+\fw,\ya+\fh);
    \node[anchor=north west, fill=black!88, text=white, rounded corners=1.6pt, inner xsep=2.4pt,
          inner ysep=1.7pt, font=\fontsize{6.2}{7}\selectfont\ttfamily] at (\xa+3.5,\ya+\fh-3.5)
      {\textcolor{filmred}{\textbullet}\kern1.2pt\tm\kern3.5pt};
    \node[anchor=base, text=\cc, inner sep=0pt, font=\fontsize{7.2}{8}\selectfont\bfseries]
      at (\xa+0.5*\fw,\sp+3.7) {\textls[70]{\what}};
  }
  \begin{scope}[shift={(1.4+\pad+\fw+0.5*\gap,\cy)}]
    \fill[filmyellow, draw=black!90, line width=0.6pt, line join=miter]
      (90:14) \foreach \k in {0,...,11} { -- ({105+\k*30}:8.6) -- ({120+\k*30}:14) } -- cycle;
    \fill[filmred, draw=white, line width=0.35pt, line join=miter, scale=60]
      (-0.02,0.15) -- (0.08,0.15) -- (0.03,0.03) -- (0.10,0.03) -- (-0.07,-0.16) -- (-0.02,-0.03) -- (-0.09,-0.03) -- cycle;
  \end{scope}
  \foreach \dx in {-5.8,0.8}
    \draw[filmyellow, line width=2.4pt, line cap=butt, line join=miter]
      (1.4+\pad+2*\fw+1.5*\gap+\dx,\cy+6.5) -- ++(5,-6.5) -- ++(-5,-6.5);
  \node[anchor=south west, inner sep=0pt, outer sep=0pt] at (1.4,0)
    {\href{\videoaddress}{\makebox[\dimexpr\W pt-2.8pt\relax]{\rule{0pt}{\HB pt}}}};
\end{tikzpicture}%

